On the Configurations of Closed Kinematic Chains in three-dimensional Space

A kinematic chain in three-dimensional Euclidean space consists of $n$ links that are connected by spherical joints. Such a chain is said to be within a closed configuration when its link lengths form a closed polygonal chain in three dimensions. We investigate the space of configurations, described in terms of joint angles of its spherical joints, that satisfy the the loop closure constraint, meaning that the kinematic chain is closed. In special cases, we can find a new set of parameters that describe the diagonal lengths (the distance of the joints from the origin) of the configuration space by a simple domain, namely a cube of dimension $n-3$. We expect that the new findings can be applied to various problems such as motion planning for closed kinematic chains or singularity analysis of their configuration spaces. To demonstrate the practical feasibility of the new method, we present numerical examples.

==> Savefile.tex <==
\begin{comment}
Note that diagonal lengths $L_{k-1}, L_k$ and $a_k$ are the side lengths of the triangle with vertices $f_{a^n, k} \left(\al^{k} ,  \be^{k} \right)$,  $f_{a^n, k-1} \left(\al^{k-1} ,  \be^{k-1} \right)$ and zero. As such one may interchange the roles of $L_k$ and $L_{k-1}$ in the above theorem. By doing so we observe that from \eqref{eq:lihanineq} for some $k\geq 3$, we get 
\begin{alignat*}{2}
\left|L_{k-2}-a_{k-1}\right| &\leq L_{k-1} &&\leq L_{k-2}+a_{k-1},\\
\left|L_{k-1}-a_k\right| &\leq L_k &&\leq L_{k-1}+a_k.
\end{alignat*}
as additional inequalities for the diagonals. From the latter two inequalities it follows that
\begin{align*}
L_{k-2}-a_{k-1}-a_k&\leq L_k\leq L_{k-2}+a_{k-1}+a_k,\\
-L_{k-2}+a_{k-1}-a_k&\leq L_k,\quad\text{and}\\
-L_{k-2}-a_{k-1}+a_k&\leq L_k.
\end{align*}
Consecutively combining the inequalities backwards in the same manner from $k$ to $1$, we infer the inequalities
\begin{align*}
2a_i-\sum_{j=1}^ka_k\leq L_k\leq \sum_{j=1}^ka_j,\quad 1\leq i\leq k,
\end{align*}
or, put differently, we get lower and upper overall bounds for $L_k, 1\leq k\leq n-1$
\begin{align}\label{eq:cmincmaxB}
\mathrm{    R}_{k}^{min}   :=  \max_{1\leq i\leq k}\left(2a_i-\sum_{j=1}^ka_j\right)&\leq L_k\leq \sum_{j=1}^ka_j := \mathrm{    R}_{k}^{max}   ,\quad 1\leq i\leq k.
\end{align}

\end{comment}
